ERNIE 3.0 Tiny: Frustratingly Simple Method to Improve Task-Agnostic Distillation Generalization

Task-agnostic knowledge distillation attempts to address the problem of deploying large pretrained language model in resource-constrained scenarios by compressing a large pretrained model called teacher into a smaller one called student such that the student can be directly finetuned on downstream tasks and retains comparable performance. However, we empirically find that there is a generalization gap between the student and the teacher in existing methods. In this work, we show that we can leverage multi-task learning in task-agnostic distillation to advance the generalization of the resulted student. In particular, we propose Multi-task Infused Task-agnostic Knowledge Distillation (MITKD). We first enhance the teacher by multi-task training it on multiple downstream tasks and then perform distillation to produce the student. Experimental results demonstrate that our method yields a student with much better generalization, significantly outperforms existing baselines, and establishes a new state-of-the-art result on in-domain, out-domain, and low-resource datasets in the setting of task-agnostic distillation. Moreover, our method even exceeds an 8x larger BERT$_{\text{Base}}$ on SQuAD and four GLUE tasks. In addition, by combining ERNIE 3.0, our method achieves state-of-the-art results on 10 Chinese datasets.

==> EMNLP 2022/table/table_ablation1.tex <==
\begin{table}[h]
\centering
\scalebox{0.75}{
\begin{tabular}{lcccc}
\hline
Method &
QNLI & CHEMPROT & LEDGAR & SCIREC	\\
\hline
RoBERTa$_{Large}$ & \textbf{94.7} & \textbf{86.9} & \textbf{} & \textbf{90.6} \\
Muppet$_{Base}$ & 93.3 & 83.6 & & 89.3 \\
\hline
MiniLMv2 & 90.9 & 74.5 & 86.8 & 80.3 \\
MITKD & \textbf{91.7} & \textbf{79.0} & \textbf{86.8} & \textbf{82.4} \\
\hline
\end{tabular}
}
\caption{Comparison with student distilled from a stronger teacher.\label{table:ablation1}}
\end{table}
\vspace{-2cm}


==> EMNLP 2022/table/table_data_num.tex <==
\begin{table}[h]
\centering
\scalebox{0.83}{
\begin{tabular}{lcccc}
\hline
porportion &
QNLI & CHEMPROT & LEDGAR & SCIREC	\\
\hline
1\%  & 1047 & 41 & 600 & 32\\
10\% & 10474 & 416 & 6000 & 321\\
50\%  & 52371 & 2084 & 30000 & 1609\\
\hline
\end{tabular}
}
\caption{\label{table:data_num} Number of training data.}
\end{table}


==> EMNLP 2022/table/table_domain_shift_num.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{lc}
\hline
Task &
Vocab. Overlap	\\
\hline
FinBank & 7.6\% \\
CHEMPROT & 8.5\% \\
ACL-ARC & 13.7\% \\
SCIERC & 14.5\% \\
PARTISAN & 30.8\% \\
SCOTUS & 39.4\% \\
ANLI & 39.4\% \\
PubMed & 48.1\% \\
HELPFUL & 54.2\% \\
LEDGAR & 56.0\% \\
\hline
\end{tabular}
}
\caption{Vocab. overlap between tasks in MTL and out-of-domain task.\label{table:domain_shift_num}}
\end{table}

